Neurosymbolic Architectural Reasoning: Towards Formal Analysis through Neural Software Architecture Inference

Formal analysis to ensure adherence of software to defined architectural constraints is not yet broadly used within software development, due to the effort involved in defining formal architecture models. Within this paper, we outline neural architecture inference to solve the problem of having a formal architecture definition for subsequent symbolic reasoning over these architectures, enabling neurosymbolic architectural reasoning. We discuss how this approach works in general and outline a research agenda based on six general research question that need to be addressed, to achieve this vision.

==> acronym.tex <==
\begin{acronym}[ECU]
\acro{ADT}{Alternating Decision Trees}
\acro{BN}{Bayesian Network}
\acro{CARM}{Classification Association Rule Mining}
\acro{DT}{Decision Trees}
\acro{HDP}{Hierarchical Dirichlet Process}
\acro{LDA}{Latent Dirichlet Allocation}
\acro{LLM}{Large Language Model}
\acroplural{LLM}[LLMs]{Large Language Models}
\acro{LR}{Logistic Regression}
\acro{LSTM}{Long Short-Term Memory}
\acro{MNB}{Multinomial Na\"ive Bayes}
\acro{NB}{Na\"ive Bayes}
\acro{RF}{Random Forest}
\acro{SVM}{Support Vector Machine}
\acro{TFM}{Term Frequency Matrix}
\acro{IDF}{Inverse Document Frequency}
\end{acronym}
